Deepening the Relationship between SEFE and C-Planarity

In this paper we deepen the understanding of the connection between two long-standing Graph Drawing open problems, that is, Simultaneous Embedding with Fixed Edges (SEFE) and Clustered Planarity (C-PLANARITY). In his GD'12 paper Marcus Schaefer presented a reduction from C-PLANARITY to SEFE of two planar graphs (SEFE-2). We prove that a reduction exists also in the opposite direction, if we consider instances of SEFE-2 in which the intersection graph is connected. We pose as an open question whether the two problems are polynomial-time equivalent.

==> makefile <==
finalname = main

psfiles = \


pdf:
	pdflatex $(finalname).tex



startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.out
	rm -f *.backup
	rm -f *.pdf

bib: 
	pdflatex $(finalname).tex
	bibtex $(finalname)
	pdflatex $(finalname).tex
	pdflatex $(finalname).tex

ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o



print: ps
	lpr -Ppolaris -h $(finalname).ps

